Domain Generalisation via Imprecise Learning

Out-of-distribution (OOD) generalisation is challenging because it involves not only learning from empirical data, but also deciding among various notions of generalisation, e.g., optimising the average-case risk, worst-case risk, or interpolations thereof. While this choice should in principle be made by the model operator like medical doctors, this information might not always be available at training time. The institutional separation between machine learners and model operators leads to arbitrary commitments to specific generalisation strategies by machine learners due to these deployment uncertainties. We introduce the Imprecise Domain Generalisation framework to mitigate this, featuring an imprecise risk optimisation that allows learners to stay imprecise by optimising against a continuous spectrum of generalisation strategies during training, and a model framework that allows operators to specify their generalisation preference at deployment. Supported by both theoretical and empirical evidence, our work showcases the benefits of integrating imprecision into domain generalisation.

==> content/09_discussion_notes.tex <==
{\hrule}

\subsection{Meeting summary: 13th April 2023}
\begin{itemize}
\item The distinction between natural and artificial cause for distribution shifts is misleading. Revise this sentence: Prior work has shown that the distribution can shift due to unintentional causes, such as image acquisition techniques across hospitals, change in patient populations, time, or intentional due to adversarial attacks and strategic manipulations.
\item For now, the most crucial step for us is defining the OOD problem and the uncertainty that our OOD definition inherits. From this definition, it should follow that OOD is not only a statistical inference problem but also a choice problem.
\item Prior work on OOD tackles specific forms of distribution shifts, while assuming a risk aversiveness at training time. For example, we assume that adversarial attacks will occur at test time, and we aim to very risk averse (i.e., be robust against the worst case attacks), then we have an $f^{*}$ and we know the right objective (i.e., min/max objective). In contrast, when we speak of OOD, we have assume no or little knowledge on what shift may realizes at test time. In addition, we do not want to anticipate the risk aversiveness at test time. 
\item We discussed the definition of aleatoric and epistemic uncertainty \citep{hullermeier2021} in the context of OOD. However, these ``classical'' definitions of uncertainty do not fit to our problem definition of OOD because in OOD we have an additional source of uncertainty that is we do not know how the data may shift.
\item \cite{williamsonFairnessRiskMeasures} builds the argumentation on the Knightian definition of uncertainty (i.e., outcome to which probabilities cannot be assigned), and, as a consequence, classical probability theory is not be applicable. However, in such cases the imprecise probability theory is well adopted and gives us a connection to risk measures. Until here, we do not distinguish from the work of \cite{williamsonFairnessRiskMeasures}. 
\item We talked about a statement from Simon, which vaguely stated that we have a random variable from which we cannot sample. Alen proposed a book called uncertainty theory, which seems to deal with such scenarios.
\end{itemize}

{\hrule}

{\hrule}

\subsection{Meeting summary: 5th April 2023}
\begin{itemize}
    \item Is defining a probability space over the domains $Z$ a suitable conceptual framework for out-of-domain problems? If there is a natural phenomenon underlying the domain generation, then it is kind of natural. However, when there is adversarial attack, the distribution will not be well-defined. 
    \item \Simon{[In progress:] Can't we write the first bulletpoint in more general terms:Is defining a probability space over a random variable $Z$ that represent the \textit{statistical conditions} (\citet{gorban2017}) under which we sample $(X,Y)$ a suitable conceptual framework for out-of-distribution problems?}
    \begin{itemize}
        \item \Simon{I like the example of \citet{gorban2017} for \textit{statistical conditions}: For instance, in coin-tossing experiments, statistical conditions may refer to the way of flipping the coin, the height and strength of the throw, the speed and direction of the air flow, the roughness of the surface on which the coin falls, etc. In addition, each of these items can be detailed. Considering, for example, the method of flipping, one may distinguish flat flipping, tossing with rotation, tossing over the shoulder, tossing on the floor or on the table, tossing with control of the coin position before flipping, etc. If the aggregate of all experimental conditions were completely reproduced in each experiment, the results would always be the same. But it is impossible to reproduce all conditions in this way.}
        \item \Krik{I think of it this way. In an IID setting, machine learning scientists/engineers (aka MLers) are interested in learning a true predictor $f^*$, but they only have access to a finite sample. Hence, the best they can get is an estimate $\hat{f}$. Since $\hat{f}$ is obtained from imperfect data, MLers are ``uncertain'' about whether or not $\hat{f}$ is a good approximation of $f^*$. However, MLers can deal with this source of uncertainty by collecting more data. In an OOD setting, the MLers also face with an additional source of uncertainty, namely, \emph{the environment in which the predictor $\hat{f}$ is deployed}. Why? Because of the distribution shift, adversarial attacks, and time. All of them create uncertainty for MLers. Now, the question is how should the MLers respond to this uncertainty?
            \begin{enumerate}
                \item The MLers may treat this uncertainty as if it's the same as the first one. That is, the uncertainty can be reduced by collecting data from more environments. 
                \item The MLers may treat this uncertainty as a potential risk to the learning problem (and hence to the predictor $\hat{f}$). In this case, data from more environments serve only as a tool to mitigate the risk. The risk will never disappear even when the number of environment approaches infinity, e.g., there can always be an adversary.
            \end{enumerate}
        I believe these two approaches will have different implications on the generalization guarantee of the predictor $\hat{f}$.
        }
    \end{itemize}
    \item therefore, we need to define OOD precisely, at least make a distinction between whether we can sample $Z$ or not. That will allow us to start making a distinction to when we are \textcolor{red}{making inference}~(statistics) or \textcolor{red}{making a choice}~(economics)? \Krik{I like this distinction. I think OOD problems involve not just statistical inference, but also choice under uncertainty.}
    
    \item Can we borrow arguments from imprecise probability to justify/ design our learning objective? One starting point is to treat the population risk for each domain as a gamble. Alan will investigate further and hopefully make the connections between choice theory, imprecise probability, and risk measures clearer. \Simon{Starting point for IP \citet{augustin2014}}
    \item On the other hand, we need a convincing concrete example on how delaying subjective model design choice at test time will benefit the model user. Finding such an example does not require us to have the infinite task model ready, we can simply train two models $\alpha_1$, $\alpha_2$ and find two subgroups of users that prefer one over the other and the other way round. Simon could focus a bit on finding/constructing such an example. \Krik{What about the following example? Choosing between worst-case and average-case solutions is a \emph{subjective} choice as it depends on how risk averse the decision makers, i.e., MLers, are. If the MLers commit to either the worst-case solution or average-case solution at training time, the problem will arise if the users (e.g., medical doctors) exhibit different levels of risk averseness. Our assumption here is that the users do not have sufficient resources to re-train the models.}
\end{itemize}

{\hrule}

\Krik{Ideas for the motivation on why we might want to learn $h(x,\alpha)$ instead of $f(x)$.}

\begin{itemize}
    \item \Simon{Numerous research papers have raised concerns regarding the reliability of machine learning models when relying excessively on i.i.d settings in uncertain environments. The reason is that in the traditional risk minimization framework, we make no assumption about uncertainty in the data-generating process (wrong: We do have uncertainty in the data generation process. However, we should question whether the conditions are stable under which repeat the experiments). Without any uncertainty, the natural way of aggregating the risks was to take the average. }
    \item In a non-i.i.d setting, we are facing uncertainty about the underlying data-generating process. \Simon{Usually, we make a further assumption to pinpoint this uncertainty to specific settings such as the change of domains, adversarial attacks, or time. In more general terms, we can assume a random variable to induce this uncertainty. This yields a probabilistic perspective on conventional risk minimization that has the advantage that we can consider the risk (expected loss) as a random variable. We refer to this induced uncertainty as hallucinated ambiguity.}\Alan{We didn't come up with this term so we should cite its origin.}
    \item \Simon{This probabilistic perspective allows us to encode a decision about an operator's risk adverseness into the model development, for example we assume that a conservative (risk averse) operator aims to be robust specifically to the tail of the risk distribution and we can reflect this operator's decision by taking the supremum over the risk instead of the average.}
    \item \Simon{\textbf{1\textsuperscript{st} Contribution:} We advocate for a probabilistic perspective on traditional empirical risk minimization to tackle the non-i.i.d setting, and we formulate the risk averseness as a decision problem on how we aggregate the risks. From this formulation, we can recover specific problem settings such as domain generalization, adversarial attacks, fairness, and a combination thereof.}
    %\item This uncertainty involves trade-offs that are only obtainable during the deployment time. As a result, we must take this uncertainty into account during training time.
    \item \Simon{Yet, the decision on the risk aversion has to be done at training time. Given that we decided on some parameter $\alpha$ to reflect the operator's risk averseness at training time, we aim to find $h_{\alpha}(x)$}.
    \item An operator of the model during deployment time can exhibit different levels of confidence about the environments in which the model is operating.  Training data are no longer available during deployment time. Even then the data are available, it may be too costly to retrain the model.
    \item \Simon{\textbf{2\textsuperscript{nd} Contribution:} We present an approach that allows to decide on the risk-aversion at test-time by learning a function $h(x,\alpha)$.}
    \item Learning $h(x,\alpha)$ will enable the model to be adaptive to the confidence/conservativeness level of its operator.
    \item Different applications may require different degrees of risk. The model that can adapt to varying degrees of risk-averseness can be more trustworthy when deployed in the real world. 
\end{itemize}

==> content/extra.tex <==
%Consider that $h$ is the Pareto optimal point for $\{\rho_{\alpha_1}[\cR](h),\dots, \rho_{\alpha_N}[\cR](h)\}$
%and that for the local gradients of objectives at $h$ the $rank(\{v{\alpha_i}\}_{i=1}^N)=N$. Then there exists a convex combination of local gradients which is equal to zero.  
%\begin{equation}
%    \sum_{i=1}^Nq_iv_{\alpha_i}=0, q_i\geq 0, \sum_{i=1}^Nq_i=1
%\end{equation}
%Equivalently $0\in Convexhull(\{v_{\alpha_i}\}_{i=1}^N)$. Consider at $h$ an additional objective $\rho_{\alpha_{N+1}}[\cR](h)$, $v_{{\alpha}_{N+1}}$ the local gradient at $h$. Since $v_{{\alpha}_{N+1}}\in \RR^N$, it can be written as a linear combination of $\{v_{\alpha_i}\}_{i=1}^N$. 
%\begin{equation}
%  v_{{\alpha}_{N+1}}=\sum_{i=1}^N a_i v_{\alpha_i}
%\end{equation}
%Given that $h$ is pareto optimal for N objectives. For $h$ to be pareto-optimal for $\rho_\Theta=\{\rho_{\alpha_1}[\cR](h),\dots, \rho_{\alpha_{n=N+1}}[\cR](h)\}$, there should not exist $w\in \RR^N$ such that $\rho_{\alpha_{N+1}}[\cR](h_-\epsilon w)<\rho_{\alpha_{N+1}}[\cR](h)$ and for $i\in \{1,\dots, N\}$ $\rho_{\alpha_{i}}[\cR](h_-\epsilon w)\leq\rho_{\alpha_{i}}[\cR](h)$.\\~\\
%Assume that, $h$ is not pareto-optimal for $\rho_\Theta$, then there exists such $w\in \RR^N$ such that $\rho_{\alpha_{N+1}}[\cR](h_-\epsilon w)<\rho_{\alpha_{N+1}}[\cR](h)$ and for $i\in \{1,\dots, N\}$ $\rho_{\alpha_{i}}[\cR](h-\epsilon w)\leq\rho_{\alpha_{i}}[\cR](h)$.\\
%Which would mean $v_{{\alpha}_{N+1}}^Tw>0$ and $v{\alpha_i}^Tw\geq 0$ for $i\in \{1,\dots, N\}$. Since $v_{{\alpha}_{N+1}}$ is linearly dependent on $\{v_{\alpha_i}\}_{i=1}^N$, $\exists i$ such that $v_{\alpha_i}^Tw\neq 0$. Since $w\in \RR^N$ exists, $v_{\alpha_i}^Tw>0$ which results in a contradiction that $h$ is pareto optimal for $\{v_{\alpha_i}\}_{i=1}^N$. Hence $h$ should be pareto optimal for $\rho_\Theta$. We can then expand the $Convexhull(\{v_{\alpha_i}\}_{i=1}^N)$ to include $v_{{\alpha}_{N+1}}$. Since $0\in Convexhull(\{v_{\alpha_i}\}_{i=1}^N)$, for the expanded convex hull, $0\in Convexhull(\{v_{\alpha_i}\}_{i=1}^{N+1})$.\\~\\
Given the case of infinite objectives, the objectives are indexed by $\alpha\in\Theta$. For $h$ they can be written as $\rho_\alpha[R](h)$. If the input space $\Theta$ is a Locally Compact Hausdorff Space we can define a positive definite kernel $k:\Theta\times\Theta\rightarrow\RR$ as:
\begin{equation}
    K(\alpha, \alpha')=v_\alpha(h)^Tv_\alpha'(h)
\end{equation}
Where $v_\alpha(h)=\nabla\rho_\alpha[\cR](h)$. Then we can show that if $h$ is C-Pareto Optimal it is C-Pareto Stationary. Consider a mapping specific to point $h$ as $L_{h}: q\rightarrow \EE_{\alpha\sim q}[v_\alpha(h)]$ where $q$ is a probability density and $\EE_{\alpha\sim q}[v_\alpha(h)]\in \cH$. If we can show that $k$ is not a characteristic kernel at $h$, the mapping $L_{h}$ is not injective. This means that there exists a probability density $q$ such that $L_{h}(q)=0$. 
\begin{proof}
    We prove this with contradiction. Assume that $h$ is Pareto optimal point and kernel $k$ is characteristic. Since $k$ is characteristic it is also conditionally strictly positive definite kernel. A kernel is (conditionally) strictly pd. if for any $n\in \NN (n\geq2)$ and $b_1,\dots,b_n\in \RR$, ($\sum_{i=1}^nb_i=0$) and $\alpha_1, \dots, \alpha_n\in \Theta$
    \begin{equation}
        \sum_{i,j=1}^n b_ib_jk(\alpha_i, \alpha_j) \geq 0
    \end{equation}
    For strictness, the equality is only true when ($b_1=b_2=\dots=b_n=0$). However for a finite $n\geq n_p+1$ we can write can obtain the equality for kernel $k$ with non trivial $b_i$'s.
    \begin{align*}
        \sum_{i,j=1}^n b_ib_jv_{\alpha_i}(h)^Tv_{\alpha_j}(h) = 0 \\
        \bigg[\sum_{i=1}^n b_iv_{\alpha_i}(h)\bigg]^T\bigg[\sum_{j=1}^nb_jv_{\alpha_j}(h)\bigg]=0
    \end{align*}
    We can obtain the equality by setting $b_i$'s as the linear coefficients for $\{v_{\alpha_i}\}_{i=1}^{n}$ since $rank(\{v_{\alpha_i}\}_{i=1}^{n})=n_p$. Therefore for finitely many parameters, this results in a contradiction since strictness does not hold for kernel $k$. Therefore it cannot be characteristic and there exists a probability density $q$ such that $L_h(q)=0$.
\end{proof}
\subsection{Proof of Proposition ~\ref{prop:nplusonefromn}}
\begin{proof}
    Let $h_\beta$ be Pareto optimal for $n_p+1$ objectives with local gradients $\{v_{\alpha_i}(h_\beta)\}_{i=1}^{n_p+1}$. We assume that $\text{rank}(\{v_{\alpha_i}(h_\beta)\}_{i=1}^{n_p+1})=n_p$ and $\text{dim}(v_{\alpha_i}(h_\beta))=n_p$. This means that a subset of $n_p$ out of $n_p+1$ local gradients span the parameter space. 

    
    Assume that $h_\beta$ is not Pareto optimal for $n_o>n_p+1$ objectives. Then there exists $h_{\beta'}\succ h_\beta$ for $n_o>n_p+1$ objectives. This means that $\rho_{\alpha_i}[\cR](h_{\beta'})\leq \rho_{\alpha_i}[\cR](h_\beta)$ for all $i\in \{1,\dots, n\}$ and there exists $\tilde{\alpha}$ such that $\rho_{\tilde{\alpha}}[\cR](h_{\beta'})< \rho_{\tilde{\alpha}}[\cR](h_\beta)$. 

    
    Now the only possible setting is that $\tilde{\alpha}\in\{\alpha_{n_p+2},\dots,\alpha_{n_o}\}$ and for $\alpha_i\in\{\alpha_1,\dots, \alpha_{n_p+1}\}$, $\rho_{\alpha_i}[\cR](h_{\beta'})=\rho_{\alpha_i}[\cR](h_\beta)$. 
    Otherwise $h_\beta$ will not be Pareto optimal for $n_p+1$ objectives. Then, from Remark ~\ref{remark:dotw}, we can conclude that there exists $w$ such that $w^{\top}v_{\tilde{\alpha}}(h_\beta)>0$. 
    And simultaneously $w^{\top}v_{\alpha_{i}}(h_\beta)=0$ for all $\alpha_i\in\{\alpha_1,\dots, \alpha_{n_p+1}\}$. 
    Since $dim(v_{\alpha_i}(h_\beta))=n_p$, then for any $\tilde{\alpha}$ we can represent $v_{\tilde{\alpha}}(h_\beta)$ as linear combination of $n_p$ independent local gradients. Without loss of generality assuming a permutation of first $n_p$ gradients to be independent at $h_\beta$. Then we can write
    \begin{equation*}
        w^{\top}v_{\tilde{\alpha}}(h_\beta) = \sum_{i=1}^{N} a_i w^{\top}v_{\alpha_i}(h_\beta) > 0,
    \end{equation*}
    where $a_i$'s are the coefficients of the linear combination. This means that $w^{\top}v_{\alpha_i}(h_\beta)\neq0$ for an   
    $\alpha_i \in\{\alpha_1,\dots, \alpha_{n_p}\}$, which contradicts our assumption that $w^{\top}v_{\alpha_{i}}(h_\beta)=0$ for all $\alpha_i\in\{1,\dots, n_p+1\}$. Hence $h_{\beta'}\nsucc h_\beta$ and $h_\beta$ is Pareto optimal for $n_o\geq n_p+1$ objectives.
\end{proof}
\subsection{Denseness of Pareto optimal solutions}
Consider $n_o$ to be the number of objectives and $\Theta_{n_o}=\{\alpha_1,\dots,\alpha_{n_o}\}$ and $n_p$ is number of parameters. Now $B_{n_o}=\{\beta\in \RR^{n_p}| h_\beta \text{ is Pareto Optimal w.r.t } \Theta_{n_o}\}$. We iteratively add objectives, therefore $\Theta_{n_o+1}=\Theta_{n_o}\cup \{\alpha_{n_o+1}\}$ and correspondingly define $B_{n_o+1}$. Analogously, $B_\infty=\{\beta\in\RR^{n_p}| h_{\beta}\text{ is C-Pareto Optimal w.r.t } \Theta_{\infty}=[0,1]\}$. \\~\\
Similar to set of pareto optimal solutions we also define the set of pareto stationary solutions as $S_{n_o}=\{\beta\in\RR^{n_p}| \exists q_i\geq 0, \sum_{i=0}^{n_o} q_i=1 \sum_{i=0}^{n_o} q_i v_{\alpha_i}(h_\beta)=0\}$. Where $v_\alpha(h_\beta):=\nabla_\beta \rho_\alpha[R](h_\beta)$. Is the set of pareto stationary points for $\Theta_{n_o}$ objectives. Similar to $B_\infty$ we also define $S_\infty=\{\beta\in\RR^{n_p}| h_{\beta} \text{ is C-Pareto Stationary w.r.t } \Theta_{\infty}=[0,1]\}$.
\begin{proposition}
    $S_1\subseteq S_2 \subseteq \dots \subseteq S_\infty$
    \label{prop:snoplusone}
\end{proposition}
\begin{proof}
    Consider objectives $\Theta_{n_o}$ and $\Theta_{n_o+1}$ such that $\Theta_{n_o}\subseteq\Theta_{n_o+1}$. The set of pareto stationary points for the objectives is given as $S_{n_o}$ and $S_{n_o+1}$ respectively. For all $\beta \in S_{n_o}$, $\beta\in S_{n_o}+1$. since $\exists q$ such that $q_i\geq 0, \sum_{i=0}^{n_o} q_i=1, \sum_{i=0}^{n_o} q_i v_{\alpha_i}(h_\beta)=0$. Where we can now construct $q'$ such that $q'_i=q_i$ for all $i \in {1,\dots,n_o}$ and $q_i=0$ for $i=n_o+1$. 
\end{proof}
Now if we assume that $\forall \alpha\in \Theta_\infty$ $\rho_\alpha[R](h)$ is convex in $h$. Then $S_{n_o}=B_{n_o}$ for all $n_o$. Thus $B_1\subseteq B_2 \subseteq \dots \subseteq B_\infty$. 
\begin{proposition}
    There exists a $N\in \NN$ such that for all $n_o\geq N$, $B_{n_o}$ is dense in $B_\infty$ given the function of objectives across $\alpha$ i.e. $\rho_\alpha[R](h)$ can be smoothly approximated by $\rho'_\alpha[R](h)=\sum_{i=0}^{n_o}w_iK(\alpha,\alpha_i)$, where $K:\Theta_\infty\times\Theta_\infty\rightarrow\RR_+$ is a kernel and $w=K(\Theta_{n_o},\Theta_{n_o})^{-1}\rho_{\Theta_{n_o}}$.  
\end{proposition}
Here $\rho_{\Theta_{n_o}}$ is a vector of fixed $\Theta_{n_o}$ atoms of objectives and is defined as, $[\rho_{\Theta_{n_o}}]_i=\rho_{\alpha_i}[R](h)$. Equivalently we can also write the smooth approximation as 
\begin{align*}
    \rho'_\alpha[R](h) = K(\alpha,\Theta_{n_o})^TK(\Theta_{n_o},\Theta_{n_o})^{-1}\rho_{\Theta_{n_o}}
\end{align*}
\begin{proof}
    We need to show that $\overline{B}_{n_o}=B_\infty$. From Proposition~\ref{prop:snoplusone} that $B_{n_o}\subseteq B_\infty$ given that $\rho_\alpha[R](h)$ is convex in $h$. We also know that $\overline{B}_{n_o}=\overline{S}_{n_o}=S_{n_o}$ and $B_\infty=S_\infty$. Therefore, We need to only need to show that $S_\infty\subseteq S_{n_o}$. Consider a $\beta\in S_\infty$ for which there must exist a probability density $q$ such that 
    \begin{align*}
        \EE_{\alpha\sim q}[v_{\alpha}(h_\beta)]=0
    \end{align*}
    Given that $\rho_\alpha[R](h)$ can be smoothly approximated by $\rho'_\alpha[R](h)$. Therefore $v_{\alpha}(h_\beta)$ can be replaced by $\nabla_{\beta}\rho'_{\alpha}(h_\beta):=K(\alpha,\Theta_{n_o})^TK(\Theta_{n_o},\Theta_{n_o})^{-1}\nabla_\beta\rho_{\Theta_{n_o}}$, where $[\nabla_\beta\rho_{\Theta_{n_o}}]_i=v_{\alpha_i}(h_\beta)$.
    \begin{align*}
        \EE_{\alpha\sim q}[\nabla_{\beta}\rho'_{\alpha}(h_\beta)]&=0\\
        \int\displaylimits_{\alpha\in\Theta_{\infty}}K(\alpha,\Theta_{n_o})^TK(\Theta_{n_o},\Theta_{n_o})^{-1}\nabla_\beta\rho_{\Theta_{n_o}}q(\alpha)\,d\alpha &= 0\\
        \int\displaylimits_{\alpha\in\Theta_{\infty}}{\nabla_\beta\rho_{\Theta_{n_o}}}^TK(\Theta_{n_o},\Theta_{n_o})^{-1}K(\alpha,\Theta_{n_o})q(\alpha)\,d\alpha &= 0\\{\nabla_\beta\rho_{\Theta_{n_o}}}^TK(\Theta_{n_o},\Theta_{n_o})^{-1}\int\displaylimits_{\alpha\in\Theta_{\infty}}K(\alpha,\Theta_{n_o})q(\alpha)\,d\alpha &= 0\\
        {\nabla_\beta\rho_{\Theta_{n_o}}}^Tq'_{\Theta_{n_o}}=0
    \end{align*}
Where $q'_{\Theta_{n_o}}:=K(\Theta_{n_o},\Theta_{n_o})^{-1}\int\displaylimits_{\alpha\in\Theta_{\infty}}K(\alpha,\Theta_{n_o})q(\alpha)\,d\alpha$. $q'_{\Theta_{n_o}}$ is a vector of all positive coefficients since $K$ is a kernel and $q$ is a probability density. Therefore normalizing $q'_{\Theta_{n_o}}$ shows that $\beta\in S_{n_o}$.
\end{proof}

%\begin{proposition}
%    $B_1,B_2,\dots, B_\infty$ are open sets 
%\end{proposition}
%\begin{proof}
%    Consider for $n_o$ objectives the corresponding set $B_{n_o}$. For $B_{n_o}$ to be an open set, there exists an $\epsilon>0$ $\forall \beta \in B_{n_o}$ such that $\cB_{\epsilon}(\beta)\subseteq B_{n_o}$. Where $\cB_\epsilon(\beta)={\beta'\in \RR^{n_p}|||\beta'\beta||_2<\epsilon}$.\\
%    Let $\beta'\in \cB_\epsilon(\beta)$ such that $\beta'-\beta=\gamma$ and $||\gamma||_2<\epsilon$. Then for all $\alpha\in \Theta_{n_o}$
%    \begin{align*}
%        \rho_\alpha[R](h_\beta')=\rho_\alpha[R](h_\beta)+\gamma^Tv_\alpha(h_\beta)+\cO(\epsilon^2)
%    \end{align*}
%    Now for $\beta'\not\in B_{n_o}$, $\rho_\alpha[R](h_\beta')\leq \rho_\alpha[R](h_\beta)$ for all $\alpha\in \Theta_{n_o}$ and there exists an $\tilde{\alpha}\in \Theta_{n_o}$ for which the inequality is strict. Which implies that 
%    \begin{align*}
%        \rho_\alpha[R](h_\beta')&\leq rho_\alpha[R](h_\beta)\\
%        \gamma^Tv_\alpha(h_\beta)+\cO(\epsilon^2) &\leq 0
%    \end{align*}
%    For no open ball to exist the above condition must be true for all $\epsilon>0$. However for sufficiently small $\epsilon$, 
%    \begin{align*}
%        \gamma^Tv_\alpha(h_\beta)&\leq 0
%    \end{align*}
%    Which is in contradiction to Remark ~\ref{remark:dotw} of our proposition ~\ref{prop:existsw}. Hence $\beta'\in B_{n_o}$.
%\end{proof}

\paragraph{Future direction}

\begin{itemize}
    \item Can we show that we can learn $h(x,\alpha)$? How would we learn $h(x,\alpha)$?
    \item Next step: Look together with Anurag into multi-objective optimization (MOO) literature. In MOO, we have to include $\alpha$ somehow in the function $f$, for example, as an additional feature.
\end{itemize}

\paragraph{Some references for Anurag}

\begin{itemize}
    \item Sener, O. and Koltun, V. (2018). Multi-task learning as multi-objective optimization. NeurIPS 2018.
    \item Pareto Navigation Gradient Descent: a First-Order Algorithm for Optimization in Pareto Set
    \item Debabrata Mahapatra and Vaibhav Rajan. Multi-task learning with user preferences: Gradient descent with controlled ascent in pareto optimization. In International Conference on Machine Learning, 2020.
    \item Mohammad Mahdi Kamani, Rana Forsati, James Z Wang, and Mehrdad Mahdavi. Pareto efficient fairness in supervised learning: From extraction to tracing. arXiv:2104.01634, 2021.
    \item Shuxiao Chen, Koby Crammer, Hangfeng He, Dan Roth, and Weijie J Su. Weighted training for cross-task learning. arXiv:2105.14095, 2021.
    \item Xi Lin, Hui-Ling Zhen, Zhenhua Li, Qingfu Zhang, and Sam Kwong. Pareto multi-task learning. arXiv:1912.12854, 2019.
    \item Pingchuan Ma, Tao Du, and Wojciech Matusik. Efficient continuous pareto exploration in multi-task learning. In International Conference on Machine Learning, 2020.
    \item Timo M Deist, Monika Grewal, Frank JWM Dankers, Tanja Alderliesten, and Peter AN Bosman. Multi-objective learning to predict pareto fronts using hypervolume maximization. arXiv:2102.04523, 2021.
    \item Aviv Navon, Aviv Shamsian, Gal Chechik, and Ethan Fetaya. Learning the pareto front with hypernetworks. arXiv:2010.04104, 2020.
    \item Xi Lin, Zhiyuan Yang, Qingfu Zhang, and Sam Kwong. Controllable pareto multi-task learning. arXiv:2010.06313, 2020.
    \item Multi-task learning as a bargaining game. ICML 2022.
\end{itemize}
\textbf{Lemma 1 in finite objective setting}\\~\\
Consider concurrent optimization for a finite set of choices $\Theta=\{\alpha_1,\dots,\alpha_n\}$ which induce the corresponding set of objectives $\rho_{\Theta}=\{\rho_{\alpha_1}[\cR](h),\dots, \rho_{\alpha_n}[\cR](h)\}$ which are smooth functions of $h$. At a point $h_\beta$ we can write the local gradient for objective $\rho_{\alpha_i}[\cR](h)$ as $u_i=\nabla_\beta\rho_{\alpha_i}[\cR](h_\beta)$. We assume that the gradients belong to $\RR^N$. $h_\beta$ is a pareto-optimal point with respect to $\rho_{\Theta}$ if there exists a convex combination of $\{u_i\}_{i=1}^n$ that equals to 0. 
\begin{equation}
    \sum_{i=1}^nq_iu_i=0, q_i\geq 0, \sum_{i=1}^nq_i=1
\end{equation}
\begin{proof}
\textbf{Case1: $n_o\leq n_p$}\\~\\ 
Let $r$ be the rank of the family of gradients $r=rank(\{v_{\alpha_i}\}_{i=1}^{n_o})=dimSp(\{v_{\alpha_i}\}_{i=1}^{n_o})$ and let us examine the different possible cases of $r$.\\
If $r=0$ all the gradients are equal to zero and rest is trivial. 
if $r=1$ the gradient-vectors are colinear say $v_{\alpha_i}=\lambda_i w$, where $w$ denotes some unit vector and the coefficients $\lambda_i$'s are not all equal to zero. Then a perturbation vector $-\epsilon w$ for sufficiently small $\epsilon>0$ cause $\delta \rho_\alpha[R](h_\beta)=-\epsilon w+ \cO(\epsilon^2)$. Thus if all coefficients $\lambda_i$ were of same sign, say positive, then at least one criterion would diminish while others would remain unchanged up to $\cO(\epsilon^2)$, and this would contradict that $h$ is pareto-optimal. Hence, necessarily both strictly positive and negative coefficients are present, and maybe some are equal to zero. Assume for example, $\lambda_i\lambda_j<0$ and then $\kappa_1=-\frac{\lambda_1}{\lambda_1-\lambda_2}, \kappa_2=\frac{\lambda_1}{\lambda_1-\lambda_2}$ so that $\kappa_1>0, \kappa_2>0$ and $\kappa_1+\kappa_2=1$, $v_{\alpha_1}\kappa_1+v_{\alpha_2}\kappa_2=0$. 
\\~\\
If $2\leq r \leq n_o-1$. Possibly after a permutation of indices, a linear combination of the first $r+1 (r+1\leq n_o)$ gradient vectors is equal to zero. 
\begin{equation}
    v_{\alpha_1}+\sum_{k=2}^{r+1}\mu_k v_{\alpha_k}=0
\label{eq:case2finitenlessthanN}
\end{equation}
Then we claim that $\mu_k\geq 0 (\forall k\geq 2)$. To establish this, assume instead that $\mu_2<0$ and define $V=Sp(\{v_{\alpha_i}\}_{i=3}^{r+1})$. Then $dim V\leq r-1 \leq n_o-2 \leq n_p-2$ and $dim V^\perp\geq 2$. Let $w\in V^\perp$, then taking the scalar product of Eq \ref{eq:case2finitenlessthanN} with $w$ gives following:
\begin{equation}
    v_{\alpha_1}^Tw = \frac{-1}{\mu_2}v_{\alpha_2}^Tw
\end{equation}
If above relation were a trivial equality ($0=\frac{-1}{\mu_2}\times 0$) for all $w\in V^\perp$ then $v_{\alpha_1},v_{\alpha_2}\in V$, so whole family $\{v_{\alpha_i}\}_{i=1}^{n_o}$ could be in $V$, which would have rank $r$ by assumption. However the $dim V\leq r-1$. Hence for some $w\in dim V^\perp$, $v_{\alpha_1}^Tw\neq 0$. Suppose for example $v_{\alpha_1}^Tw\geq 0$. Then an $\epsilon>0$ perturbation in the direction of $-w$ would improve $\rho_{\alpha_1}[\cR]$ and $\rho_{\alpha_2}[\cR]$ while keeping other objectives unchanged. This would be in contradiction to $h$ being pareto optimal. Hence $\mu_2>0$ and therefore, $\mu_k\geq 0 (\forall k\geq 2)$. Then we can define $q_i=\frac{\mu_i}{\sum_{i=1}^{n_o}\mu_i}$.\\~\\
If $r=n_o$ and $\rho_{\alpha_i,h_\beta}=\rho_{\alpha_i}[\cR](h_\beta)$. Then for all $\alpha_i$, $h$ is the solution of following minimization problem subject to inequality constraints.
\begin{equation}
    min_{\tilde{h}}\rho_{\alpha_i}[\cR](\tilde{h})\quad s.t. \text{ }\text{ } g_k(\tilde{h}):=\rho_{\alpha_j}[\cR](\tilde{h})-\rho_{\alpha_i,h}\leq 0 \text{ }(\forall k\neq i)
\end{equation}
Assume $i=1$ w.l.o.g. Hence, the lagrangian $L=\rho_{\alpha_i}[\cR](\tilde{h})+\sum_{k=2}^{n_o}\lambda_kg_k(\tilde{h})$, where $\lambda_k$'s are the lagrange multipliers is stationary at $\tilde{h}=h$:
\begin{equation}
    v_{\alpha_i}+\sum_{k=2}^{n_o}\lambda_k v_{\alpha_k}=0
\label{eq:requalnfinite}
\end{equation}
Given the sign conventions, Lagrange multipliers $\lambda_k$ are non-negative and when $g_k<0$, it equals zero. Instead note how Eq:\ref{eq:requalnfinite} contradicts the hypothesis $r=n_o$, which we have to reject. Therefore $r\leq n_p-1$ and all possible cases are examined.
\\~\\
\textbf{Case $n_o\geq n_p+1$:}\\~\\
The proof of cases $r=0$, $r=1$ and $2\leq r \leq n_p -1$ follows directly from setting where $r=0$, $r=1$ and $2\leq r\leq n_o-1$ when $n_o\leq n_p$. Therefore we consider the case where $r=n_p$. For a point $h_\beta$ that is Pareto optimal for $n_p+1$ objectives we can write the pareto stationarity as 
\begin{equation}
    \sum_{i=1}^{n_p+1}q_iu_i=0, q_i\geq 0, \sum_{i=1}^{n_p+1}q_i=1
\label{eq:proofnplusone}
\end{equation}
From proposition ~\ref{prop:nplusonefromn} we can say that $h_\beta$ is also pareto optimal for $n_o\geq n_p+1$ and we can extend the equation~\ref{eq:proofnplusone} to $n_o$ objectives by setting $\{q_i\}_{i=n_p+2}^{n_o}=0$ then, 
\begin{equation}
    \sum_{i=1}^{n_o}q_iu_i=0, q_i\geq 0, \sum_{i=1}^{n_o}q_i=1
\end{equation}
\end{proof}

\textbf{Lemma 1 in infinite objective setting}
%\begin{proposition}
%    If $h_\beta$ is Pareto optimal for $n_p+1$ objectives where $\text{rank}(\{{v_{\lambda_i}}(h_\beta)\}_{i=1}^{n_p+1})=n_p$ and $\text{dim}(v_{\lambda_i}(h_\beta))=n_p$, then it is Pareto optimal for $n_o\geq n_p+1$ objectives. 
%    \label{prop:nplusonefromn}
%\end{proposition}
%In Proposition ~\ref{prop:nplusonefromn} we consider the case of under-parameterization in a finite parameters setting. Given that we have $n_p$ parameters since $dim(v_{\lambda_i}(h_\beta))=n_p$, the proposition illustrates once a point is Pareto optimal for $n_o=n_p+1$ objectives it remains Pareto optimal for $n_o\geq n_p+1$. The intuition for the proposition is that at a Pareto optimal point $h_0$ where the set of gradients for the objectives span the complete parameter space, one cannot find a direction of Pareto improvement that does not depend on the set. This implies that for infinitely many objectives we can obtain a subset of the Pareto front by obtaining the front for $n_p+1$ objectives. This also serves as an important fact in proof of Lemma ~\ref{lemma:optimalityimpliesstationarity} for the case of under-parameterization in finite parameters setting.
%While the Proposition ~\ref{prop:anydistributionhstar} in theory says that any distribution as long as it has sufficient support over $\Lambda$ result in a $q^*$ that is Almost-sure C-Pareto Optimal to $h^*$ i.e. $h^*\nsucc_{P_{\lambda}}q*$. In practice, the expectation over $\lambda\in \Lambda$ is approximated by taking $n$ random samples of $\{\lambda_{i}\}_{i=1}^n\sim P_\lambda$ which results in the random function $q_n$ and the variance of this $q_n$ is affected by the choice of $P_\lambda$. 
%If we consider the overall loss incurred by $q_n$ which is the model obtained from minimizing the empirical risk
%\begin{equation}
%    q_n = arg\min_{q \in C(\cX\times\Lambda)}\sum_{i=1}^n\rho_{\lambda_i}(q(\cdot,\lambda_i))
%\end{equation}
%Then the estimation and approximation error can be decomposed as
\begin{align*}
    \EE_{\lambda\sim P_\lambda}[(\rho_{\lambda}(q_n(\cdot,\lambda)-\rho_{\lambda}(h^*(\cdot,\lambda))^2]\\\leq \EE_{\lambda\sim P_\lambda}[(\rho_{\lambda}(q_n(\cdot,\lambda)-\rho_{\lambda}(q^*(\cdot,\lambda))^2]\\+\EE_{\lambda\sim P_\lambda}[\rho_{\lambda}(q^*(\cdot,\lambda)-\rho_{\lambda}(h^*(\cdot,\lambda)]^2
\end{align*}
\section{Anurag suggested formulation}

\subsection{Describe your model}
To learn $\bar{h}:\cX\times\Theta\to\cY$ directly we use a proxy $\alpha'\sim \mathcal{U}[0,1]$ and $h(\cdot, \alpha'):\cX\to\cY$. 
 \begin{align}
        \mathcal{L}(h(\cdot,\alpha')) = \int_{0}^1 CVaR_\alpha(\TT_{h(\cdot, \alpha')}) w(\alpha,\alpha') d\alpha \quad 
    \end{align}
    where $\quad CVaR_\alpha(\TT_{h(\cdot, \alpha')}) := \EE_{R\sim \TT_{h(\cdot, \alpha')}}[R \mid R \geq F^{-1}_{\TT_{h(\cdot, \alpha')}}(\alpha)]$ is the conditional value-at-risk. And $w(\alpha,\alpha')$ is equivalent to attention/convolution over $CVaR$ objectives induced by $\alpha$ or kernel which can be fixed or learned during the optimization. 
And $\forall \alpha\in[0,1]$ and $f:\cX\to\cY$
\begin{align}
    h^*(\cdot,\alpha) = arg\min_{f} \mathcal{L}(f) 
\end{align}
\subsection{Describe what question you have in mind? What could go wrong?}
\begin{itemize}
    \item How sensitive is the optimization to the sampling of $\alpha'$.
    \item If we freely parameterize the $w(\alpha,\alpha')$ we can make the problem arbitrarily easy.  
\end{itemize}
\subsection{How to verify this method?}
We can verify the method by seeing if it does single objective optimization by setting $w(\alpha,\alpha')=\delta(\alpha,\alpha')$.\\
\textbf{Evaluation:} Following the protocol from Probable domain generalization via Quantile Risk Minimization to evaluate the method, we perform the inference on test environments and build a test risk distribution to evaluate $h(\cdot, \alpha)$ for a particular $\alpha$ but to collectively quantify performance of $h$ is still unclear. 
\subsection{Preliminary Experiments}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{content/Figures/pytorch_1/datasplit_linear.png}
    \caption{Generated data, train, and val}
    \label{fig:linear-datasplit-pytorch}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{content/Figures/pytorch_1/linear_f_linear_h_linear_theta.png}
    \caption{Risk distribution with respect to $\alpha$ for linear $f$ and linear $h$ on validation data, we consider Normal distribution based weighting $\mathcal{N}(\alpha',\alpha')$}
    \label{fig:linear-datasplit-pytorch}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{content/Figures/pytorch_1/linear_f_linear_h_nonlinear_theta.png}
    \caption{Risk distribution with respect to $\alpha$ for linear $f$ and nonlinear $h$ on validation data, we consider Normal distribution based weighting $\mathcal{N}(\alpha',\alpha')$}
    \label{fig:linear-datasplit-pytorch}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{content/Figures/pytorch_1/weighting_comparison.png}
    \caption{Risk distribution with respect to $\alpha$ on validation data, we consider Normal distribution based weighting $\mathcal{N}(\alpha',1)$ and $\mathcal{N}(\alpha',\alpha')$ on left and right respectively}
    \label{fig:linear-datasplit-pytorch}
\end{figure}
\subsubsection{Justification of objective of $h^*$}
We justify the choice of our objective for each $h(\cdot, \alpha)=argmin_{f}\mathcal{L}_{\alpha}(\mathcal{R}(f))$ using the concept of regret~\cite{}. The maximal regret in the case of statistical decision function (SDF) is defined for a planner with respect to the planner's choice and how that choice affects the welfare across different states. For a choice $c\in C$ in set of choices the planner can make, state $s\in S$ among the set of possible states, and a welfare objective $w:C\times S \rightarrow \mathbb{R}$, the choice that minimizes the maximal regret can be written as:
\begin{equation}
    \min_{c\in C}\max_{s\in S}[\max_{d\in C}w(d,s)-w(c,s)]
\end{equation}

In our problem setting, we consider starting from $\cH = \{h \mid \cX\times \Theta \to \cY\}$ to construct a state-dependent choice set $\cH=C_\Theta$ for our problem. We define the welfare analogously as $w : C_\Theta \times \Theta \to \RR$ as $w(h,\alpha)=-CVaR(h(\cdot,\alpha),\alpha)$. With the rationale that this is the welfare a practitioner obtains from $h$ with his given choice $\alpha$ from the returned augmented hypothesis. We can then generalize the concept of minimizing maximal regret in our problem as:
\begin{align}
    r &= \min_{c \in C_\Theta} \max_{\alpha \in \Theta}[\min_{d\in C_\Theta}w(d,\alpha)-w(c,\alpha)]\\
      &= \min_{h \in \cH} \max_{\alpha \in \Theta}\underbrace{[ CVaR(h(\cdot, \alpha)) - \min_{h'\in \cH}CVaR(h'(\cdot, \alpha),\alpha)]}_{:=X(h,\alpha)}
\end{align}
Considering a $\cF_{\cH,\alpha} = \{f | f:= h(\cdot, \alpha)$ s.t. $ \forall h\in\cH\}$, we can rewrite $X(h,\alpha)$ as 
\begin{align}
    X(h,\alpha) &= CVaR(h(\cdot, \alpha)) - \min_{f'\in \cF_{\cH,\alpha}}CVaR(f',\alpha)
\end{align}
Now considering the regret for $h^*$ in state $\alpha$
\begin{align}
    X(h^*,\alpha) &=  CVaR(h^*(\cdot,\alpha),\alpha)-\min_{\cF_{\cH,\alpha}} CVaR(f',\alpha)\\
    &= \min_{f\in \cF_{\cH,\alpha}}CVaR(f,\alpha)-\min_{\cF_{\cH,\alpha}} CVaR(f',\alpha)\\
    &= 0
\end{align}


\subsection{Comparison of Learners}

\subsection{Learning with Augmented Hypotheses}
To further institutionalize the separation of statistical decision making i.e. making a choice under ambiguity which is performed by the user from statistical learning which is performed by the user. We propose to learn an \emph{augmented} hypothesis $\bar{h}:\cX\times\Lambda\to\cY$ from an extended hypothesis space $\widetilde{\mathcal{H}}$ such that
\begin{equation}
    \bar{h}(x,\lambda) = h_{\lambda}^*(x) = \arg\min_{h\in\mathcal{H}}\, \rho_{\lambda}[\bm{\cR}](h)
\end{equation}

\begin{definition}[C-Pareto optimal]\label{def:pareto-optimality-2}
The augmented hypothesis $\bar{h}$ dominates $\bar{h}'$, denoted by $\bar{h} \succ \bar{h}'$, if $\rho_{\lambda}[\bm{\cR}](\bar{h}(\cdot,\lambda)) \leq \rho_{\lambda}[\bm{\cR}](\bar{h}'(\cdot,\lambda))$ for all $\lambda\in\Lambda$ and $\rho_{\tilde{\lambda}}[\bm{\cR}](\bar{h}(\cdot,\tilde{\lambda})) < \rho_{\tilde{\lambda}}[\bm{\cR}](\bar{h}'(\cdot,\tilde{\lambda}))$ for some $\tilde{\lambda}\in\Lambda$. Then, $\bar{h}$ is C-Pareto optimal if there exists no $\bar{h}'\in\widetilde{\cH}$ such that $\bar{h}' \succ \bar{h}$.
\end{definition}
\begin{assumption}
    Let $C(\cX\times\Lambda)$ be spaces of continuous functions on $\cX\times\Lambda$ and that $\bar{h}\in C(\cX\times\Lambda)$.
    \label{assume:augmented_h_continuity}
\end{assumption}
\begin{proposition}
Under the assumption~\ref{assume:augmented_h_continuity} suppose there exists a continuous function $h^*(x,\lambda)$ such that for every $\lambda\in\Lambda$, the function $h^*(\cdot,\lambda)$ obtains the bayes optimal model. Then, if $g^* \in C(\cX\times\Lambda)$ is C-Pareto optimal with respect to Definition \ref{def:pareto-optimality-2}, $g^*(\cdot,\lambda)$ also obtains the bayes optimal model for all $\lambda\in\Lambda$.
    \label{prop:uniquenessofh}
\end{proposition}
The proposition ~\ref{prop:uniquenessofh} illustrates that all C-Pareto Optimal augmented hypotheses can simultaneously learn all the Bayes optimal models given assumpition~\ref{assume:augmented_h_continuity}. In theory, a learner can perform multi-objective optimization to obtain C-Pareto optimal $g^*$. However learners can also use a distribution $P_\lambda$ to perform an aggregation over all objectives and obtain a single objective for optimization. This aggregation can be performed by taking an expectation over objectives with respect to $P_\lambda$. Therefore, every distribution corresponds to a choice of aggregation. In proposition~\ref{prop:anydistributionhstar} we illustrate that all choices of aggregation ($P_\lambda$) lead to almost sure C-Pareto optimality with respect to the choice of aggregation. 

%\Krik{The representation theorem of the dominance relation and expected risk.}

\begin{proposition}
    Under the assumption~\ref{assume:augmented_h_continuity} let $C(\cX)$ and $C(\cX\times\Lambda)$ be spaces of continuous functions on $\cX$ and on $\cX\times\Lambda$, respectively. Consider a distribution $P_\lambda$ over the choices $\Lambda$ as the aggregator of objectives $\rho_\lambda$ and the corresponding aggregated optimization problem 
    \begin{equation}\label{eq:avg_prob}
        \min_{q\in C(\cX\times\Lambda)}\EE_{\lambda\sim P_\lambda}[\rho_\lambda(q(\cdot,\lambda))]
    \end{equation}
    Let  $q^*(x,\lambda)$ be a continuous function that solves the problem ~\eqref{eq:avg_prob}, then $q^*$ also obtains bayes optimal solution for every $\lambda\in\Lambda$ such that $P(\lambda)>0$ i.e. $q^*\succeq_{P_\lambda} \bar{h}$ and $\bar{h}\succeq_{P_\lambda} q^*$.  
    \label{prop:anydistributionhstar}
\end{proposition}
The proposition states that any choice of distribution for aggregations works to learn the bayes optimal models learned for different $\lambda$ under the support of the distribution. Therefore, it indicates that under any choice of aggregation amongst distributions with full support, $q^*$ can learn $\bar{h}$ i.e. all the Bayes optimal models simultaneously, assuming that $h^*_\lambda$ are unique minimizers and continuous in $\lambda$ for every $x\in \cX$. 
\begin{table*}[]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline 
         $\lambda$ & GT ($\lambda$ known) & Median & Avg$(\lambda=0)$ & Worst$(\lambda=1)$ & Uniform $\lambda, f$ & Imprecise (Infinite-Task)\\
         \hline 
         0.0 & $\mathbf{0.209\pm 9.38e-03}$ & $0.345\pm 4.23e-02$ & $\mathbf{0.209\pm 3.60e-03}$ & $0.247\pm 6.78e-03$ & $0.235\pm 5.17e-03$ & $\mathbf{0.209\pm 6.00e-04}$\\
         0.1 & $\mathbf{0.230\pm 1.10-06}$ & $0.382\pm 4.65e-02$ & $0.230\pm 3.66e-03$ &$0.271\pm 6.93e-03$ & $0.259\pm 5.69e-03$&$0.230\pm 1.07e-03$\\
         0.3 & $\mathbf{0.267\pm 2.45e-07}$ & $0.489\pm 6.10e-02$&$0.271\pm 4.75e-03$ & $0.310\pm 7.44e-03$&$0.295\pm 7.19e-02$&$0.269\pm 1.38e-03$\\
         0.5 & $\mathbf{0.297\pm 2.62e-08}$& $0.681\pm 8.79e-02$&$0.327\pm 8.30e-03$&$0.321\pm 8.00e-03$&$0.308\pm 7.23e-02$&$\mathbf{0.296\pm 5.22e-05}$\\
         0.7 & $\mathbf{0.316\pm 1.34e-08}$& $1.039\pm 1.26e-02$&$0.455\pm 1.74e-02$&$0.326\pm 8.18e-03$&$0.319\pm 5.06e-02$&$0.318\pm 1.10e-03$\\
         0.9 & $\mathbf{0.325\pm 4.33e-03}$& $1.231\pm 1.40e-01$&$0.577\pm 2.10e-02$&$0.333\pm 7.17e-03$&$0.341\pm 1.14e-02$&$0.327\pm 2.92e-03$\\
         0.999 & $\mathbf{0.343\pm 4.33e-03}$&$1.297\pm 1.51e-01$&$0.614\pm 2.57e-02$&$\mathbf{0.343\pm 5.91e-03}$&$0.363\pm 1.34e-02$&$0.351\pm 1.07e-02$\\
         \hline 
    \end{tabular}
    }
    \caption{Comparison of Precise and Imprecise Learners}
    \label{tab:Learners}
\end{table*}
\begin{table*}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
         \hline 
         $\lambda$ & GT ($\lambda$ known) & Two stage regressor& Unif(0,1)$h$ & Beta(0.1,0.2) & Chebyshev \\
         \hline
         0.0 & $\mathbf{0.2090\pm 9.38e-03}$&$0.2094\pm 4.88e-04$& $0.2098\pm 9.72e-03$ & $0.2090\pm1.49e-04$&$0.2096\pm6.01e-04$ \\
         0.1 & $\mathbf{0.2301\pm 1.10-06}$ &$0.2300\pm 7.53e-05$& $0.2307\pm 5.03e-04$ & $0.2301\pm1.38e-04$&$0.2306\pm6.44e-04$\\
         0.3 & $\mathbf{0.2679\pm 2.45e-07}$&$0.2683\pm 2.82e-04$& $0.2696\pm 1.03e-03$ &$0.2683\pm4.54e-04$&$0.2695\pm6.87e-04$\\
         0.5 & $\mathbf{0.2970\pm 2.62e-08}$&$0.2968\pm 1.44e-04$& $0.2968\pm 1.66e-04$ & $0.2983\pm1.78e-03$&$0.2967\pm 3.58e-05$\\
         0.7 & $\mathbf{0.3164\pm 1.34e-08}$&$0.3191\pm 1.68e-03$& $0.3181\pm 1.44e-03$ & $0.3248\pm5.92e-03$&$0.3184\pm1.58e-03$\\
         0.9 & $\mathbf{0.3258\pm 4.33e-02}$&$0.3427\pm 2.49e-02$& $0.3278\pm 1.62e-02$ & $0.3344\pm8.84e-02$&$0.3271\pm1.18e-02$\\
         0.999 & $\mathbf{0.3433\pm 4.33e-02}$&$0.3735\pm 3.59e-02$& $0.3511 \pm 7.73e-02$ & $0.3440\pm6.01e-02$&$0.3432\pm2.13e-02$\\
         \hline 
    \end{tabular}
    \caption{Comparison of Choice of Distribution of $\mathbb{P}_\alpha$ over preferences $\Theta$ for Imprecise Learners}
\end{table*}
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{content/Figures/comparison/precisevsimprecise.pdf}
        \caption{}
        \label{fig:figure1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{content/Figures/comparison/ablation_p_lambda_full.pdf}
        \caption{}
        \label{fig:figure2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{content/Figures/comparison/ablation_zoomed.pdf}
        \caption{}
        \label{fig:figure3}
    \end{subfigure}
    \caption{Evaluation of Precise and Imprecise Learners. Figure (a) tries to evaluate precise and imprecise learners with $CVaR$ for various $\lambda\in\Lambda$. A learner dominates other learner it performs similar or better for all $\lambda\in\Lambda$. Figure (b) illustrates the effect of choice of $\mathbb{P}_\lambda$ for imprecise learners. Figure (c) zooms into the higher risk averseness region of Figure (b).}
    \label{fig:eval_under_continuity_assumption}
\end{figure*}
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{content/Figures/comparison/non_linear_comparison/env.pdf}
        \caption{Training Data from 250 domains}
        \label{fig:figure1}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{content/Figures/comparison/non_linear_comparison/precisevsimprecise.pdf}
        \caption{Precise vs Imprecise Learners ($m=20$)}
        \label{fig:figure2}
    \end{subfigure}
    \caption{Evaluation of Precise and Imprecise Learners. Figure (a) Denotes the training data for our simulation setup across 250 domains with 100 examples from every domain. The data generating process is $y=\theta^TX$, and $X\sim\mathcal{N}(0,1)$, $\theta=[Unif(-1.1,-1)]^{\mathbb{I}[p=1]}[Unif(1,1.1)]^{\mathbb{I}[p=0]}$ where $p\sim Bernoulli(0.8)$. Figure (b) tries to evaluate precise and imprecise learners with $CVaR$ for various $\lambda\in\Lambda$, Here we evaluate monto carlo estimate with $m=20$. A learner dominates other learner it performs similar or better for all $\lambda\in\Lambda$.}
    \label{fig:eval_under_continuity_assumption}
\end{figure*}
\begin{figure*}[ht]
    \centering
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{content/Figures/comparison/non_linear_comparison/full_plot_5.pdf}
        \caption{Choice of $P_\lambda$ for Imprecise Learners ($m=5$)}
        \label{fig:figure2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{content/Figures/comparison/non_linear_comparison/m20.pdf}
        \caption{Choice of $P_\lambda$ for Imprecise Learners ($m=20$)}
        \label{fig:figure3}
    \end{subfigure}
    \caption{Ablation of Imprecise Learners with respect to $P_\lambda$. Figure (a) Here we evaluate monte carlo estimate with $m=5$.  Figure (c) $m=20$.}
    \label{fig:eval_under_continuity_assumption}
\end{figure*}
\subsection{Simulating data generation}
To establish that choice of $P_\lambda$ which aggregates the objectives to obtain ~\eqref{eq:aggregate-with-p-lambda} imposes preference over augmented hypothesis $\tilde{\cH}$ we need to ensure that $h^*\not\in C(\cX\times\Lambda)$. Here $h^*$ is the augmented hypothesis such that $h^*(\cdot, \lambda)$ is bayes optimal for each $\lambda\in \Lambda$. For example 
\[
h^*(x,\lambda) = 
\begin{cases} 
f_{easy}(x) & , \mathbf{1}[\lambda \leq 0.5]\\
f_{hard}(x) & \mathbf{1}[\lambda>0.5].
\end{cases}
\]
Given $\lambda,\bm{\cR}$ we can obtain the weight vector $\bm{w}$ that aggregates the risk profile i.e. $\rho_\lambda[\bm{\cR}]=\sum_{i=1}^n w_i^{\lambda}\cR_i$. We can use this $\bm{w}$ to sample from the corresponding distribution in credal set.\\
However, this risk profile itself depends on $h\in \cH$. Is it possible to compute weights from this "bayes" risk profile functional $\bm{\cR}^*=(\cR_{1},\cdots,\cR_{n})$? Where for probability distribution $\mathbb{P}_i\in\cP_0$, the risk is $\cR_{i}(h^*)$ and $h^*(x)=\mathbb{E}[Y|X=x]$? Consider a random variable from empirical risk profile as $\bm{R}\sim \frac{1}{m}^\top \delta_{\bm{\cR}}$, We know that $r_\lambda = \operatorname{VaR}_\lambda(\bm{R})$, then we can show that $\operatorname{CVaR}_\lambda$ corresponds to 
\begin{align}
    \rho_\lambda[\bm{\cR}](h)   &= \sum_{i=1}^n w^{(\lambda)}_i \cR_i(h) \\
                        &= \sum_{i=1}^n \left(d_\lambda \mathbb{I}[R_i = r_\lambda] + \frac{(1-d_\lambda)}{\sum_{i=1}^n \mathbb{I}[R_i \geq r_\lambda]} \right)\cR_i(h)\\
                        &= \mathbb{E}_{\sum_{i=1} w^{(\lambda)}_i\mathbb{P}_i}[\ell(h(x),y)]
\end{align}
Assume the same setting as in Experiment 1c but now with 2 dimension input and 2 dimension in parameters with non-linear output $Y=e^{\sqrt{\theta^T X}}$, we simulate different environments by drawing $\theta$ from a uniform distribution $\ \mathcal{U}(0,1)$. In total, we generate for 25 environments 100 observations each.
\begin{figure*}[h!]
    \caption{Results of experiment 1c in one dimension.}
     \centering
     \begin{subfigure}{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/non_linear_op_1d/2d_theta_hats.png}
         \caption{Generated data and the estimated regression function $f_{\alpha}(\hat{\theta})$ for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_linear_uniform_data}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/non_linear_op_1d/2d_contour_theta.png}
         \caption{Landscape of the objective function $\rho$, specifically we picked CVaR as the aggregation function and plot $\hat{\theta}$ as circles.}
         \label{fig:1d_linear_uniform_landscape}
     \end{subfigure}
     \begin{subfigure}{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/non_linear_op_1d/2d_dist_risks.png}
        \caption{Distribution of the Risk for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_uniform_beta_risk}
     \end{subfigure}
\end{figure*}


\paragraph{Experiment 2A:} Assume a linear model $Y_{e}=\theta_{e}X+\epsilon$, where $X \sim \mathcal{N}(2,0.2)$ and $\epsilon\sim \mathcal{N}(0,0.1)$. We simulate different environments by drawing $\theta$ from a beta distribution $Beta(0.1,0.2)$. In total, we generate for 25 environments 100 observations each. For $\alpha\in[0,1]$ discretized to step size of 0.05 we run a multiobjective optimization using NSGA-2 and obtain 222 $\hat{\theta}$ on the Pareto front for 1 d linear and 254 for 1d non linear case. 

\begin{figure*}[h!]
    \caption{Results of Experiment 2A.}
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/multiob_plot.png}
         \caption{Generated data and the estimated regression function $f_{\alpha}(\hat{\theta})$ for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_linear_beta_multiobj}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/multiob_risk.png}
         \caption{Distribution of the Risk for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_linear_beta_multi_risk}
     \end{subfigure}
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/multiob_nonlinear_plot.png}
         \caption{Generated data and the estimated regression function $f_{\alpha}(\hat{\theta})$ for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_nonlinear_beta_multiobj}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/mutliobj_risk.png}
         \caption{Distribution of the Risk for $\alpha \in \{0.05, \dots, 0.95\}$ in 1-D non-linear case.}
         \label{fig:1d_nonlinear_beta_multi_risk}
     \end{subfigure}
\end{figure*}

Assume the same setting as in Experiment 1c but now with 2 dimension input and 2 dimension in parameters with non-linear output $Y=e^{\sqrt{\theta^T X}}$, we simulate different environments by drawing $\theta$ from a uniform distribution $\ \mathcal{U}(0,1)$. In total, we generate for 250 environments 10000 observations each.
\begin{figure*}[h!]
    \caption{Results of experiment 1c' in one dimension.}
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/alpha_0.05/2d_theta_alpha.png}
         \caption{Landscape of the change of $\theta$ in 2d as $\alpha$ changes}
         \label{fig:1d_linear_uniform_landscape}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/alpha_0.05/3d_theta_alpha.png}
         \caption{Landscape of the change of $\theta$ in 3d as $\alpha$ changes}
         \label{fig:1d_linear_uniform_landscape}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/alpha_0.05/risk.png}
        \caption{Distribution of the Risk for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_uniform_beta_risk}
     \end{subfigure}
\end{figure*}

Assume the same setting as in Experiment 1c but now with 2 dimension input and 2 dimension in parameters with non-linear output $Y=e^{\sqrt{\theta^T X}}$, we simulate different environments by drawing $\theta$ from a uniform distribution $\ \mathcal{U}(0,1)$. In total, we generate for 25 environments 1000 observations each.
\begin{figure*}[h!]
    \caption{Results of experiment 1c' in one dimension.}
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/alpha_0.05/2d_theta_alpha_25_1k.png}
         \caption{Landscape of the change of $\theta$ in 2d as $\alpha$ changes}
         \label{fig:1d_linear_uniform_landscape}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/alpha_0.05/3d_theta_alpha_25_1k.png}
         \caption{Landscape of the change of $\theta$ in 3d as $\alpha$ changes}
         \label{fig:1d_linear_uniform_landscape}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/29-06-23/alpha_0.05/risk_25_1k.png}
        \caption{Distribution of the Risk for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_uniform_beta_risk}
     \end{subfigure}
\end{figure*}
\paragraph{Conclusion of the simulation experiment}
\begin{itemize}
    \item Given that the operator at test time have a risk averseness between "less risk averse" and "risk averse" and by having $h(x, \alpha)$ we can cover this spectrum of the operator's risk averseness.
    \item The point is that we do not make any assumptions on the test environment, but on the ML operator's risk aversness.
    \item Learning $\theta$ based on the ARM objective with $\rho$ being CVaR works for the linear and non-linear case. However, when $f$ becomes non-linear in the output, we have to deal with a non-convex optimization, which fails in the current implementation.
\end{itemize}
\paragraph{Experiment 1B:} Assume the same setting as in Experiment 1, however, in contrast, we simulate different environments by drawing $\theta$ from a uniform distribution $\ \mathcal{U}(0,1)$. In total, we generate for 25 environments 100 observations each.

\begin{figure*}[h!]
    \caption{Results of experiment 1B.}
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/2023-05-26_uniform_1D_linear_function.pdf}
         \caption{Generated data and the estimated regression function $f_{\alpha}(\hat{\theta})$ for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_linear_uniform_data}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/2023-05-26_uniform_1D_linear_landscape.pdf}
         \caption{Landscape of the objective function $\rho$, specifically we picked CVaR as the aggregation function and plot $\hat{\theta}$ as circles.}
         \label{fig:1d_linear_uniform_landscape}
     \end{subfigure}
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/2023-05-26_uniform_1D_linear_risk_distribution.pdf}
        \caption{Distribution of the Risk for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_uniform_beta_risk}
     \end{subfigure}
\end{figure*}

In contrast to Experiment 1B, $\theta$ is sampled from a uniform distribution $\ \mathcal{U}(0,1)$. As a result, we do not observe any clusters across the environments in Figure \ref{fig:1d_linear_uniform_data}. \textbf{Question: If the environments are uniformly distributed, what implications does this have for the distribution of $R$? And why does changing $\alpha$ does not affect $f_{\alpha}(\hat{\theta})$}?

Furthermore, the landscape of the objective function is shown in Figure \ref{fig:1d_linear_uniform_landscape}. In contrast to Experiment 1A, changing $\alpha$ does not affect the optimal solution much, and the task itself seems to be similarly difficult across $\alpha$. Also, $\hat{\theta}$ is quite similar across all $\alpha$. Lastly, in Figure \ref{fig:1d_uniform_beta_risk}, the distribution of $R$ has a similar shape across all $\alpha$.

%\Simon{ToDo... 1D Non-linear case}
\paragraph{Experiment 1C:} Assume the same setting as in Experiment 1 but now non-linear in output and parameters $Y=e^{\theta X}$, we simulate different environments by drawing $\theta$ from a uniform distribution $\ \mathcal{U}(0,1)$. In total, we generate for 25 environments 100 observations each.
\begin{figure}[h!]
    \caption{Results of experiment 1c in one dimension.}
     \centering
     \begin{subfigure}[b]{0.4\linewidth}
         \centering
         \includegraphics[width=\linewidth]{content/Figures/non_linear_op_1d/regression.png}
         \caption{Generated data and the estimated regression function $f_{\alpha}(\hat{\theta})$ for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_linear_uniform_data}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\linewidth}
         \centering
         \includegraphics[width=\linewidth]{content/Figures/non_linear_op_1d/contour_of_alpha.png}
         \caption{Landscape of the objective function $\rho$, specifically we picked CVaR as the aggregation function and plot $\hat{\theta}$ as circles.}
         \label{fig:1d_linear_uniform_landscape}
     \end{subfigure}
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/Figures/non_linear_op_1d/dist_of_risks.png}
        \caption{Distribution of the Risk for $\alpha \in \{0.05, \dots, 0.95\}$.}
         \label{fig:1d_uniform_beta_risk}
     \end{subfigure}
\end{figure}


==> content/related-work.tex <==
\subsection{Previous Work}

\begin{itemize}
    \item OOD and domain generalization
        \begin{itemize}
            \item Invariance principle is necessary, but not sufficient. Heterogeneity!
            \item Ivariant Risk Minimization (IRM) and some follow-up work: Finding feature representation that leads to Bayes optimal models across all environments.
        \end{itemize}
    \item Precise vs imprecise learning
    \item Imprecise probability in machine learning
        \begin{itemize}
            \item Quantification of Credal Uncertainty in Machine Learning: A Critical Analysis and Empirical Comparison
            \item Aleatoric and Epistemic Uncertainty with Random Forests
            \item 
        \end{itemize}
    \item Test-time adaptation
    \item Meta-learning
    \item Multi-objective optimization and multi-task learning 
    \item Parametric task learning and infinite task learning
    \item Statistical decision making (Wald 19XX)
    \item etc
\end{itemize}
